Full Abstraction for the Resource Lambda Calculus with Tests, through Taylor Expansion

We study the semantics of a resource-sensitive extension of the lambda calculus in a canonical reflexive object of a category of sets and relations, a relational version of Scott's original model of the pure lambda calculus. This calculus is related to Boudol's resource calculus and is derived from Ehrhard and Regnier's differential extension of Linear Logic and of the lambda calculus. We extend it with new constructions, to be understood as implementing a very simple exception mechanism, and with a "must" parallel composition. These new operations allow to associate a context of this calculus with any point of the model and to prove full abstraction for the finite sub-calculus where ordinary lambda calculus application is not allowed. The result is then extended to the full calculus by means of a Taylor Expansion formula. As an intermediate result we prove that the exception mechanism is not essential in the finite sub-calculus.

==> include/fig0.tex <==
\begin{figure}[t]
\centering
\textbf{The big picture}\\[-2ex]
$$
\begin{tikzpicture}
  \matrix [column sep=2cm]
  {
    \node (dzl) {$\dzlam$-calculus}; & \node{}; & \node (dzlt) {$\dzlam$-calculus with tests}; \\
    \node{};&&\\
    \node{};&&\\    
    \node (te1) {};&\node (lam) {\lam-calculus};&\\        
    \node{};&&\\
    \node{};&&\\    
    \node (dl) {$\dlam$-calculus}; & \node{}; & \node (dlt) {$\dlam$-calculus with tests}; \\
  };
        \draw[->,line width=1pt] (dzl) to (dzlt) {};
        \draw[->,line width=1pt] (dzl) to (dl) {};   
        \draw[->,line width=1pt] (dl) to (dlt) {};
        \draw[->,line width=1pt] (lam) to (dl) {};                
        \draw[->,line width=1pt] (lam) to (dlt) {};        
        \draw[->,line width=1pt] (dzlt) to (dlt) {}; 
        \draw[->,dashed,line width=1pt] (dl) to[out=180,in=180] (dzl) {};       
        \draw[->,dashed,line width=1pt] (dlt) to[out=0,in=0] (dzlt) {};               
        \draw[->,dotted,line width=1pt] (dzlt) to[out=166,in=15] (dzl) {};                       
        \node at (7.2,0) {$\TE{(\cdot)}$};
        \node at (-7.2,0) {$\TE{(\cdot)}$};        
        \node at (-0.5,2.1) {\footnotesize test-expansion};                
\end{tikzpicture}
$$
\caption{\footnotesize Relationships among calculi. Solid arrows stand for injections, dashed arrows for Taylor expansion, the dotted arrow for test-expansion.}
\label{fig:calculi}
\end{figure}

==> include/preliminaries.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Preliminaries}\label{sec:preliminaries}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{\bf Sets and modules.}\label{subs:sets} 
We denote by $\nat$ the set of natural numbers and by $\one$ an arbitrary singleton set. Given a set $S$, we write $\Pow{S}$ (resp.\ $\Powf{S}$) for the set of all
 (resp.\ all finite) subsets of $S$. Given $k\in\nat$, we denote by $\perm{k}$ the \emph{set of all permutations of $\{1,\ldots,k\}$}.

Let $\bool$ be the semiring $\{0,1\}$ with $1+1=1$ and multiplication defined in the obvious way. For any set $S$, we write $\bool\langle S \rangle$ for the free
 $\bool$-module generated by $S$, so that $ \bool\langle S \rangle\cong\Powf{S}$ with addition corresponding to union, and scalar multiplication defined in the
 obvious way. However we prefer to keep the algebraic notations for elements of $\bool\langle S \rangle$, hence set unions will be denoted by $+$ and the empty set
 by $0$.

\subsection{\bf Multisets.}\label{subs:msets} 
Let $S$ be a set. A \emph{multiset} $a$ over $S$ can be defined as an unordered list $a = [\ga_1,\ga_2,\ldots]$ with repetitions such that $\ga_i\in S$ for all
 indices $i$. A multiset $a$ is called \emph{finite} if it is a finite list; we denote by $\card a$ its cardinality. We write $\Mfin{S}$ for the set of all finite
 multisets over $S$. Given two multisets $a = [\ga_1,\ga_2,\ldots]$ and $b = [\gb_1,\gb_2,\ldots]$ the \emph{multiset union} of $a,b$ is defined by
 $a\mcup b = [\ga_1,\gb_1,\ga_2,\gb_2,\ldots]$. Given two finite sequences of multisets $\seq a,\seq b$ of the same length $n$ we define
 $\seq a\mcup\seq b = (a_1\mcup b_1,\ldots,a_n\mcup b_n)$.

